You Drive Me Crazy! Interactive QoE Assessment for Telepresence Robot Control

Telepresence robots (TPRs) are versatile, remotely controlled vehicles that enable physical presence and human-to-human interaction over a distance. Thanks to improving hardware and dropping price points, TPRs enjoy the growing interest in various industries and application domains. Still, a satisfying experience remains key for their acceptance and successful adoption, not only in terms of enabling remote communication with others, but also in terms of managing robot mobility by means of remote navigation. This paper focuses on the latter aspect of remote operation which has been hitherto neglected. We present the results of an extensive subjective study designed to systematically assess remote navigation Quality of Experience (QoE) in the context of using a TPR live over the Internet. Participants were 'beamed' into a remote office space and asked to perform characteristic TPR remote operation tasks (driving, turning, parking). Visual and control dimensions of their experience were systematically impaired by altering network characteristics (bandwidth, delay and packet loss rate) in a controlled fashion. Our results show that users can differentiate well between visual and navigation/control aspects of their experience. Furthermore, QoE impairment sensitivity varies with the actual task at hand.

==> tables/ratings.latex <==
% latex table generated in R 3.5.3 by xtable 1.8-4 package
% Tue Jan 21 22:44:06 2020
\begin{table}[ht]
\centering
\begin{tabular}{rrrllll}
  \hline
 & Fval.q1 & Fval.q2 & pval.q1 &  & pval.q2 &  \\ 
  \hline
bw & 22.850 & 101.652 & $<$0.001 & *** & $<$0.001 & *** \\ 
  delay & 57.007 & 3.468 & $<$0.001 & *** & 0.02 & * \\ 
  plr & 13.872 & 56.450 & $<$0.001 & *** & $<$0.001 & *** \\ 
  task & 5.834 & 1.236 & 0.006 &   & 0.292 &   \\ 
  iter & 0.221 & 2.066 & 0.926 &   & 0.094 &   \\ 
   \hline
%\end{tabular}
%\end{table}
% latex table generated in R 3.5.3 by xtable 1.8-4 package
% Tue Jan 21 22:44:06 2020
%\begin{table}[ht]
%\centering
%\begin{tabular}{rrrllrl}
%  \hline
 & Chi.q1 & Chi.q2 & pval.q1 &  & pval.q2 &  \\ 
  \hline
bw:userid & 10.689 & 9.947 & 0.001 &   & 0.002 &   \\ 
  delay:userid & 2.859 & 4.584 & 0.091 &   & 0.032 & * \\ 
  plr:userid & 0.182 & 8.340 & 0.669 &   & 0.004 &   \\ 
  task:userid & 3.225 & 0.000 & 0.073 &   & 0.999 &   \\ 
  iter:userid & 13.992 & 6.341 & $<$0.001 & *** & 0.012 & * \\ 
  userid & 1.512 & 4.830 & 0.219 &   & 0.028 & * \\ 
   \hline
\end{tabular}
\caption{Fixed and Random Effects for q1, q2} 
\label{tab:mm_anova}
\end{table}

